A Robust Adversarial Network-Based End-to-End Communications System With Strong Generalization Ability Against Adversarial Attacks

We propose a novel defensive mechanism based on a generative adversarial network (GAN) framework to defend against adversarial attacks in end-to-end communications systems. Specifically, we utilize a generative network to model a powerful adversary and enable the end-to-end communications system to combat the generative attack network via a minimax game. We show that the proposed system not only works well against white-box and black-box adversarial attacks but also possesses excellent generalization capabilities to maintain good performance under no attacks. We also show that our GAN-based end-to-end system outperforms the conventional communications system and the end-to-end communications system with/without adversarial training.

==> related_work.tex <==
\section{Related Work}
\label{sec:rel_work}
In this section, we overview recent literature focusing on performing adversarial attacks for deep learning based communications systems and also discuss the existing method for defending against adversarial attacks.

\subsection{Adversarial Attacks on Deep Learning Based Communications Systems}

~\cite{sadeghi2019physical}
~\cite{sadeghi2018adversarial}
~\cite{kim2020over}
~\cite{Liu2020AdversarialAO}



\newpage

\subsection{Defensive Methods Against Adversarial Attacks}
~\cite{kurakin2017adversarial}
~\cite{Wang2019ICLR}

\newpage



